An Analysis of Datasets, Metrics and Models in Keyphrase Generation

Keyphrase generation refers to the task of producing a set of words or phrases that summarises the content of a document. Continuous efforts have been dedicated to this task over the past few years, spreading across multiple lines of research, such as model architectures, data resources, and use-case scenarios. Yet, the current state of keyphrase generation remains unknown as there has been no attempt to review and analyse previous work. In this paper, we bridge this gap by presenting an analysis of over 50 research papers on keyphrase generation, offering a comprehensive overview of recent progress, limitations, and open challenges. Our findings highlight several critical issues in current evaluation practices, such as the concerning similarity among commonly-used benchmark datasets and inconsistencies in metric calculations leading to overestimated performances. Additionally, we address the limited availability of pre-trained models by releasing a strong PLM-based model for keyphrase generation as an effort to facilitate future research.

==> figures/measure/abs-f5.tex <==
\begin{axis}[
    ybar,
    bar width=12pt,
    enlarge x limits=0.3,
    width=8cm,
    height=3cm,
    ymin=0,
    ymax=10,
    ymajorgrids=true,
    grid style={dash pattern=on \pgflinewidth off 1pt, black!15},
    xtick style={draw=none},
    ytick style={draw=none},
    ytick pos=left,
    xtick=\empty,
    nodes near coords,
    nodes near coords align={vertical},
    every node near coord/.append style={font=\tiny},
    ytick={3,6},
    yticklabels={3,\phantom{0}6},
    yticklabel style={font=\scriptsize},
    % symbolic x coords={catSeqTG,ExHiRD,SetTrans},
    % xtick=data,
    ylabel={\scriptsize \textbf{Ab} - \tiny $F_1@5$},
    ]

\addplot[draw=ori_color, fill=ori_color!50!white, text=ori_color, xshift=7pt] coordinates {(1,2.7) (2,1.6) (3,5.8)};
\addplot[draw=ours_color, fill=ours_color!50!white, text=ours_color, xshift=7pt] coordinates {(1,3.1) (2,1.9) (3,4.2)};
\addplot[draw=ours_norm_color, fill=ours_norm_color!50!white, text=ours_norm_color, xshift=7pt] coordinates {(1,3.2) (2,2.2) (3,4.0)};
\addplot[draw=ours_norm_color, fill=ours_norm_color!50!white, text=ours_norm_color, xshift=-7pt, postaction={
        pattern=north east lines
    }] coordinates {(3,4.0) };

% \addplot coordinates {(catSeqTG,2.7) (ExHiRD,1.6) (SetTrans,5.8)};
% \addplot coordinates {(catSeqTG,3.1) (ExHiRD,1.9) (SetTrans,4.2)};
% \addplot coordinates {(catSeqTG,3.2) (ExHiRD,2.2) (SetTrans,4.0)};
\end{axis}
%\draw (-0.2,0.15) node {\small 0};
\draw[sepbar] (2.2,+0.02) -- (2.2,1.45);
\draw[sepbar] (4.2,+0.02) -- (4.2,1.45);
%\node[inner sep=1pt] at (5.75, 1.28) {\scriptsize \textbf{Abs} - $F_1@5$};

\draw (1.2,-0.45) node {catSeqTG};
\draw (3.2,-0.4) node {ExHiRD};
\draw (5.2,-0.4) node {SetTrans};


%catSeqTG
%ExHiRD
%SetTrans

==> figures/measure/abs-fm.tex <==
\begin{axis}[
    ybar,
    bar width=12pt,
    enlarge x limits=0.3,
    width=8cm,
    height=3cm,
    ymin=0,
    ymax=10,
    ymajorgrids=true,
    grid style={dash pattern=on \pgflinewidth off 1pt, black!15},
    xtick style={draw=none},
    ytick style={draw=none},
    ytick pos=left,
    xtick=\empty,
    nodes near coords,
    nodes near coords align={vertical},
    every node near coord/.append style={font=\tiny},
    ytick={3,6},
    yticklabels={3,\phantom{0}6},
    yticklabel style={font=\scriptsize},
    ylabel={\scriptsize \textbf{Ab} - \tiny $F_1@M$},
    ]
\addplot[draw=ori_color, fill=ori_color!50!white, text=ori_color, xshift=7pt] coordinates {(1,5.0) (2,3.2) (3,3.6) };
\addplot[draw=ours_color, fill=ours_color!50!white, text=ours_color, xshift=7pt] coordinates {(1,5.6) (2,3.7) (3,5.7) };
\addplot[draw=ours_norm_color, fill=ours_norm_color!50!white, text=ours_norm_color, xshift=7pt] coordinates {(1,5.1) (2,3.9) (3,5.1) };

\addplot[draw=ours_norm_color, fill=ours_norm_color!50!white, text=ours_norm_color, xshift=-7pt, postaction={
        pattern=north east lines
    }] coordinates {(1,5.1) (3,5.1) };

\end{axis}
%\draw (-0.2,0.15) node {\small 0};
\draw[sepbar] (2.2,-0.05) -- (2.2,1.45);
\draw[sepbar] (4.2,-0.05) -- (4.2,1.45);
%\node[inner sep=1pt] at (5.67, 1.28) {\scriptsize \textbf{Abs} - $F_1@M$};

==> figures/measure/pres-f5.tex <==
\begin{axis}[
    ybar,
    bar width=12pt,
    enlarge x limits=0.3,
    width=8cm,
    height=3cm,
    ymajorgrids=true,
    grid style={dash pattern=on \pgflinewidth off 1pt, black!15},
    ymin=22,
    ymax=48,
    ytick style={draw=none},
    xtick style={draw=none},
    ytick pos=left,
    xtick=\empty,
    nodes near coords,
    nodes near coords align={vertical},
    every node near coord/.append style={font=\tiny},
    ytick={30,40},
    %yticklabels={30,40},
    yticklabel style={font=\scriptsize},
    ylabel={\scriptsize \textbf{Pr} - \tiny $F_1@5$},
    ]
\addplot[draw=ori_color, fill=ori_color!50!white, text=ori_color, xshift=7pt] coordinates {(1,32.1) (2,31.1) (3,39.5) };
\addplot[draw=ours_color, fill=ours_color!50!white, text=ours_color, xshift=7pt] coordinates {(1,31.6) (2,30.5) (3,33.5) };
\addplot[draw=ours_norm_color, fill=ours_norm_color!50!white, text=ours_norm_color, xshift=7pt] coordinates {(1,28.1) (2,26.9) (3,30.0) };

\addplot[draw=ours_norm_color, fill=ours_norm_color!50!white, text=ours_norm_color, xshift=-7pt, postaction={
        pattern=north east lines
    }] coordinates {(1,28.1) (2,26.9) (3,30.0) };

\end{axis}
%\draw (-0.2,0.15) node {\small 0};
\draw[sepbar] (2.2,-0.05) -- (2.2,1.45);
\draw[sepbar] (4.2,-0.05) -- (4.2,1.45);
%\node[inner sep=1pt] at (5.76, 1.28) {\scriptsize \textbf{Pre} - $F_1@5$};

==> figures/measure/pres-fm.tex <==
\pgfplotsset{compat=1.11,
    /pgfplots/ybar legend/.style={
    /pgfplots/legend image code/.code={%
       \draw[##1,/tikz/.cd,yshift=-0.25em]
        (0cm,0cm) rectangle (5pt,0.6em);},
   },
}

\begin{axis}[
    ybar,
    bar width=12pt,
    enlarge x limits=0.3,
    width=8cm,
    height=3cm,
    ymajorgrids=true,
    grid style={dash pattern=on \pgflinewidth off 1pt, black!15},
    ymin=22,
    ymax=49,
    ytick style={draw=none},
    xtick style={draw=none},
    ytick pos=left,
    xtick=\empty,
    inner frame sep=0pt,
    nodes near coords,
    nodes near coords align={vertical},
    every node near coord/.append style={font=\tiny},
    ytick={30,40},
    %yticklabels={30,40},
    yticklabel style={font=\scriptsize},
    legend style={at={(0.1,1.36)},legend columns=-1,anchor=north west,font=\footnotesize,draw=none,inner sep=1pt}, %,column sep=.3cm},
    legend cell align={center},
    %legend style={at={(0.5,1.5)}, anchor=north, legend columns=-1},
    ylabel={\scriptsize \textbf{Pr} - \tiny{$F_1@M$}},
    ]
\addlegendentry{Original\quad~}
\addplot[draw=ori_color, fill=ori_color!50!white, text=ori_color, xshift=7pt] coordinates {(1,38.6) (2,37.4) (3,35.9) };
\addlegendentry{Ours\quad~}
\addplot[draw=ours_color, fill=ours_color!50!white, text=ours_color, xshift=7pt] coordinates {(1,37.8) (2,36.6) (3,37.2) };
\addlegendentry{Ours \tiny{w/o norm.}}
\addplot[draw=ours_norm_color, fill=ours_norm_color!50!white, text=ours_norm_color, xshift=7pt] coordinates {(1,35.5) (2,34.4) (3,35.2) };

\addplot[draw=ours_norm_color, fill=ours_norm_color!50!white, text=ours_norm_color, xshift=-7pt, postaction={
        pattern=north east lines
    }] coordinates {(1,35.5) (2,34.4) (3,35.2) };


%\node[] at (axis cs: 0,1) {\footnotesize $F_1@M$};

\end{axis}
\draw[sepbar] (2.2,-0.05) -- (2.2,1.4);
\draw[sepbar] (4.2,-0.05) -- (4.2,1.4);
%\draw (-0.2,0.15) node {\small 0};
%\draw[line] (6, 1.4) node {\footnotesize $F_1@M$};
%\node[text width=1cm,inner sep=-3pt] at (6.05, 1.25) {\scriptsize $F_1@M$};
%\node[inner sep=1pt] at (5.69, 1.28) {\scriptsize \textbf{Pre} - $F_1@M$};

